The Boolean quadratic forms and tangent law

In \cite{EjsmontLehner:2020:tangent} we study the limit sums of free commutators and anticommutators and show that the generalized tangent function $$ \frac{\tan z}{1-x\tan z} $$ describes the limit distribution. This is the generating function of the higher order tangent numbers of Carlitz and Scoville \cite[(1.6)]{CarlitzScoville:1972} which arose in connection with the enumeration of certain permutations. In the present paper we continue to study the limit of weighted sums of Boolean commutators and anticommutators and we show that the shifted generalized tangent function appears in a limit theorem. In order to do this, we shall provide an arbitrary cumulants formula of the quadratic form. We also apply this result to obtain several results in a Boolean probability theory.

==> 9 V/cyr.tex <==
\usepackage[OT2,OT1]{fontenc}
\newcommand\cyr
{
\renewcommand\rmdefault{wncyr}
\renewcommand\sfdefault{wncyss}
\renewcommand\encodingdefault{OT2}
\normalfont
\selectfont
}
\DeclareTextFontCommand{\textcyr}{\cyr}
\def\cprime{\char"7E }
\def\cdprime{\char"7F }
\def\eoborotnoye{\char’013}
\def\Eoborotnoye{\char’003}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> 9 V/formulas/inneroddfig-pstricks.tex <==
  \begin{figure}[h]
\begin{center}
\vspace{1cm}
\psset{nodesep=3pt}
\psset{angle=90}

\rnode{A1}{\Node{$\star$}}\rnode{A2}{\Node{$\star$}}\rnode{A}{\Node{$\star$}} \rnode{B}{\Node{$\star$}} \rnode{C}{\Node{$\star$}}
\rnode{D}{\Node{$\star$}}
\ncbar[armA=.2]{A1}{A2}
\ncbar[armA=0.6]{A2}{A}
\ncbar[armA=.2]{A}{B}
\ncbar[armA=0.8]{A1}{B}
\ncbar[armA=0.8]{B}{C}
%\ncbar[armA=.2]{A}{B}
\ncbar[armA=.2]{C}{D} 
\hspace{6mm}
\rnode{A7}{\Node{$\star$}}\rnode{A5}{\Node{$\star$}}\rnode{A6}{\Node{$\star$}}\rnode{A3}{\Node{$\star$}}\rnode{A1}{\Node{$\star$}}\rnode{A2}{\Node{$\star$}}\rnode{A}{\Node{$\star$}} \rnode{B}{\Node{$\star$}} \rnode{C}{\Node{$\star$}}
\rnode{D}{\Node{$\star$}} \rnode{D1}{\Node{$\dots$}} \rnode{D2}{\Node{$\star$}} \rnode{D3}{\Node{$\star$}}
\ncbar[armA=.2]{A7}{A5}
\ncbar[armA=.2]{A6}{A3}
\ncbar[armA=.2]{A1}{A2}
\ncbar[armA=0.6]{A2}{A}
\ncbar[armA=0.8]{A7}{A3}
\ncbar[armA=0.6]{A6}{A5}
\ncbar[armA=0.8]{A7}{A1}
\ncbar[armA=.2]{A}{B}
\ncbar[armA=0.8]{A7}{B}
\ncbar[armA=0.8]{B}{C}
%\ncbar[armA=.2]{A}{B}
\ncbar[armA=.2]{C}{D}  
\ncbar[armA=.2]{D2}{D3}
\caption{Irreducible
%which  the property that $\pi \vee \hat{0}_{[2r]}^2=1_{[2r]}.$ 
}
\label{fig:FiguraExemple1}
\end{center}
\end{figure} 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> 9 V/formulas/involutiontypeIIIa.tex <==
%\usetikzlibrary{backgrounds}

\begin{tikzpicture}[scale=0.5]
\draw [white] (0,3.0) circle (0);

    \path [afill,thick] (2.0,0) rectangle (7.2,1.0);
\draw [thick] (0.7,0)--(0.7,1.6)--(7.9,1.6)--(7.9,0);
\draw [thick] (1.3,0)--(1.3,1.0)--(2.0,1.0);
\draw [dashed] (-1.8,1.6)--(10.3,1.6);

\node at (0.6,-0.5){$\pm X Y$};
\end{tikzpicture}

==> 9 V/formulas/involutiontypeIIIb.tex <==
%\usetikzlibrary{backgrounds}

\begin{tikzpicture}[scale=0.5]
\draw [white] (0,3.0) circle (0);
    \path [afill,thick] (1.1,0) rectangle (6.3,1.0);
\draw [thick] (0.7,0)--(0.7,1.6)--(7.9,1.6)--(7.9,0);
\draw [thick] (7.2,0)--(7.2,1.0)--(6.3,1.0);
\draw [dashed] (-1.8,1.6)--(10.3,1.6);

\node at (7.2,-0.5){$\mp Y X$};
\end{tikzpicture}

==> 9 V/formulas/minpartition1a.tex <==
%latex kernelSetPartition [1,1,2,2,1]
\begin{picture}(24,6.5)(1,0)
  \put(1,0){\line(0,1){7.5}}
  \put(6,0){\line(0,1){7.5}}
  % \put(14,0){\line(0,1){4.5}}
  % \put(20,0){\line(0,1){4.5}}
  \put(8,0){$\cdots$}
  \put(24,0){\line(0,1){7.5}}
  % \put(14,4.5){\line(1,0){6}}
  \put(6,7.5){\line(1,0){18}}
\end{picture}


==> 9 V/formulas/minpartition1b.tex <==
\begin{picture}(24,6.5)(1,0)
  \put(1,0){\line(0,1){7.5}}
  \put(18,0){\line(0,1){7.5}}
  % \put(14,0){\line(0,1){4.5}}
  % \put(20,0){\line(0,1){4.5}}
  \put(2,0){$\cdots$}
  \put(24,0){\line(0,1){7.5}}
  % \put(14,4.5){\line(1,0){6}}
  \put(1,7.5){\line(1,0){18}}
\end{picture}

==> 9 V/formulas/minpartition1e.tex <==
\begin{picture}(30,6.5)(1,0)
  \put(1,0){\line(0,1){7.5}}
  \put(6,0){\line(0,1){7.5}}
  % \put(14,0){\line(0,1){4.5}}
  % \put(20,0){\line(0,1){4.5}}
  \put(8,0){$\cdots$}
  \put(24,0){\line(0,1){7.5}}
  % \put(14,4.5){\line(1,0){6}}
  \put(6,7.5){\line(1,0){18}}
    \put(30,0){\line(0,1){7.5}}

\end{picture}

==> 9 V/formulas/notinneroddfig-pstricks.tex <==

 \begin{figure}[h]
\begin{center}
\vspace{1cm}
\psset{nodesep=3pt}
\psset{angle=90}

\rnode{A7}{\Node{$\star$}}\rnode{A5}{\Node{$\star$}}\rnode{A6}{\Node{$\star$}}\rnode{A3}{\Node{$\star$}}\rnode{A1}{\Node{$\star$}}\rnode{A2}{\Node{$\star$}}\rnode{A}{\Node{$\star$}} \rnode{B}{\Node{$\star$}} \rnode{C}{\Node{$\star$}}
\rnode{D}{\Node{$\star$}} \rnode{D1}{\Node{$\star$}} \rnode{D5}{\Node{$\star$}} \rnode{D2}{\Node{$\star$}} \rnode{D3}{\Node{$\star$}} \rnode{F1}{\Node{$\star$}} \rnode{F2}{\Node{$\star$}} \rnode{F3}{\Node{$\star$}} \rnode{F4}{\Node{$\star$}}
\ncbar[armA=.2]{A7}{A5}
\ncbar[armA=.2]{A6}{A3}
\ncbar[armA=.2]{A1}{A2}
\ncbar[armA=0.6]{A2}{A}
\ncbar[armA=0.6]{A5}{A6}
\ncbar[armA=0.6]{A3}{A1}
\ncbar[armA=.2]{A}{B}
\ncbar[armA=.2]{D1}{D5}


\ncbar[armA=1]{A7}{B}
\ncbar[armA=1]{B}{D3}
%\ncbar[armA=.2]{A}{B}
\ncbar[armA=.2]{C}{D}  
\ncbar[armA=.2]{D2}{D3}
\ncbar[armA=.2]{F1}{F2}
\ncbar[armA=.2]{F3}{F4}
\ncbar[armA=.6]{F2}{F3}
\ncbar[armA=1]{F1}{F4}
\ncbar[armA=1]{F1}{D3}

\caption{No irreducible }
\label{fig:FiguraExemple2}
\end{center}
\end{figure} 


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> 9 V/formulas/pi111222x.tex <==
\begin{picture}(32,6.5)(1,0)
   \put(0,8){\line(0,1){8}}
  \put(6,8){\line(0,1){4.5}}
  \put(12,8){\line(0,1){4.5}}
  \put(18,8){\line(0,1){8}}
  \put(24,8){\line(0,1){4.5}}
  \put(30,8){\line(0,1){4.5}}
 % \put(32,0){\line(0,1){4.5}}
 % \put(38,0){\line(0,1){4.5}}
  %\put(18,12.5){\line(1,0){12}}
  \put(0,16){\line(1,0){18}}
\end{picture}

==> 9 V/formulas/pi111222xx.tex <==
\begin{picture}(32,6.5)(1,0)
   \put(0,8){\line(0,1){4.5}}
  \put(6,8){\line(0,1){4.5}}
  \put(12,8){\line(0,1){4.5}}
  \put(18,8){\line(0,1){4.5}}
  \put(24,8){\line(0,1){4.5}}
  \put(30,8){\line(0,1){4.5}}
 % \put(32,0){\line(0,1){4.5}}
 % \put(38,0){\line(0,1){4.5}}
  %\put(18,12.5){\line(1,0){12}}
 % \put(0,16){\line(1,0){18}}
\end{picture}

==> 9 V/formulas/pi111222xxx.tex <==
\begin{picture}(32,6.5)(1,0)
   \put(0,8){\line(0,1){4.5}}
  \put(6,8){\line(0,1){4.5}}
  \put(12,8){\line(0,1){4.5}}
  \put(18,8){\line(0,1){4.5}}
  \put(24,8){\line(0,1){4.5}}
  \put(30,8){\line(0,1){4.5}}
 % \put(32,0){\line(0,1){4.5}}
 % \put(38,0){\line(0,1){4.5}}
  %\put(18,12.5){\line(1,0){12}}
  \put(6,12.5){\line(1,0){24}}
\end{picture}

==> 9 V/formulas/pi112221x.tex <==
\begin{picture}(32,6.5)(1,0)
   \put(0,8){\line(0,1){4.5}}
  \put(6,8){\line(0,1){4.5}}
  \put(12,8){\line(0,1){4.5}}
  \put(18,8){\line(0,1){4.5}}
  \put(24,8){\line(0,1){4.5}}
  \put(30,8){\line(0,1){4.5}}
 % \put(32,0){\line(0,1){4.5}}
 % \put(38,0){\line(0,1){4.5}}
  \put(18,12.5){\line(1,0){12}}
  \put(0,12.5){\line(1,0){12}}
\end{picture}

==> 9 V/formulas/pi112221xx.tex <==
\begin{picture}(32,6.5)(1,0)
   \put(0,8){\line(0,1){4.5}}
  \put(6,8){\line(0,1){4.5}}
  \put(12,8){\line(0,1){4.5}}
  \put(18,8){\line(0,1){4.5}}
  \put(24,8){\line(0,1){4.5}}
  \put(30,8){\line(0,1){4.5}}
 % \put(32,0){\line(0,1){4.5}}
 % \put(38,0){\line(0,1){4.5}}
 % \put(18,12.5){\line(1,0){12}}
  \put(0,12.5){\line(1,0){30}}
\end{picture}

==> 9 V/formulas/pi112233_1.tex <==
\begin{picture}(32,3.5)(1,0)
{
  \linethickness{\thick}
  \put(2,0){\line(0,1){4.5}}
  \put(8,0){\line(0,1){4.5}}
}
\put(14,0){\line(0,1){4.5}}
\put(20,0){\line(0,1){4.5}}
\put(26,0){\line(0,1){4.5}}
\put(32,0){\line(0,1){4.5}}
{
  \linethickness{\thick}
  \put(2,4.5){\line(1,0){6}}
}
\put(14,4.5){\line(1,0){6}}
\put(26,4.5){\line(1,0){6}}
\end{picture}

==> 9 V/formulas/pi112233_2.tex <==
\begin{picture}(32,3.5)(1,0)
\put(2,0){\line(0,1){4.5}}
\put(8,0){\line(0,1){4.5}}
{
  \linethickness{\thick}
  \put(14,0){\line(0,1){4.5}}
  \put(20,0){\line(0,1){4.5}}
}
\put(26,0){\line(0,1){4.5}}
\put(32,0){\line(0,1){4.5}}
\put(2,4.5){\line(1,0){6}}
{
  \linethickness{\thick}
  \put(14,4.5){\line(1,0){6}}
}
\put(26,4.5){\line(1,0){6}}
\end{picture}

==> 9 V/formulas/pi112233_3.tex <==
\begin{picture}(32,3.5)(1,0)
\put(2,0){\line(0,1){4.5}}
\put(8,0){\line(0,1){4.5}}
\put(14,0){\line(0,1){4.5}}
\put(20,0){\line(0,1){4.5}}
{
  \linethickness{\thick}
  \put(26,0){\line(0,1){4.5}}
  \put(32,0){\line(0,1){4.5}}
}
\put(2,4.5){\line(1,0){6}}
\put(14,4.5){\line(1,0){6}}
{
  \linethickness{\thick}
  \put(26,4.5){\line(1,0){6}}
}
\end{picture}

==> 9 V/formulas/sp0n.tex <==
%latex kernelSetPartition [1,2,3,4,5]
\begin{picture}(26,3.5)(1,0)
  \put(2,0){\line(0,1){4.5}}
  \put(8,0){\line(0,1){4.5}}
%  \put(14,0){\line(0,1){4.5}}
%  \put(20,0){\line(0,1){4.5}}
\put(10,0){$\cdots$}
  \put(26,0){\line(0,1){4.5}}
  \put(2,4.5){\line(1,0){0}}
  \put(8,4.5){\line(1,0){0}}
  \put(14,4.5){\line(1,0){0}}
  \put(20,4.5){\line(1,0){0}}
  \put(26,4.5){\line(1,0){0}}
\end{picture}

==> 9 V/formulas/sp111221a.tex <==
%latex kernelSetPartition [1,1,1,2,2,1,1]
\begin{picture}(38,6.5)(1,0)
\put(2,0){\line(0,1){7.5}}
\put(8,0){\line(0,1){7.5}}
\put(14,0){\line(0,1){7.5}}
\put(16,0){$\cdots$}
%\put(20,0){\line(0,1){4.5}}
%\put(26,0){\line(0,1){4.5}}
\put(32,0){\line(0,1){7.5}}
\put(38,0){\line(0,1){7.5}}
%\put(20,4.5){\line(1,0){6}}
\put(2,7.5){\line(1,0){36}}
\end{picture}

==> 9 V/formulas/sp1n.tex <==
%latex kernelSetPartition [1,1,2,2,1]
\begin{picture}(25,6.5)(1,0)
  \put(1,0){\line(0,1){7.5}}
  \put(6,0){\line(0,1){7.5}}
  % \put(14,0){\line(0,1){4.5}}
  % \put(20,0){\line(0,1){4.5}}
  \put(8,0){$\cdots$}
  \put(25,0){\line(0,1){7.5}}
  % \put(14,4.5){\line(1,0){6}}
  \put(1,7.5){\line(1,0){24}}
\end{picture}


==> formulas/inneroddfig-pstricks.tex <==
  \begin{figure}[h]
\begin{center}
\vspace{1cm}
\psset{nodesep=3pt}
\psset{angle=90}

\rnode{A1}{\Node{$\star$}}\rnode{A2}{\Node{$\star$}}\rnode{A}{\Node{$\star$}} \rnode{B}{\Node{$\star$}} \rnode{C}{\Node{$\star$}}
\rnode{D}{\Node{$\star$}}
\ncbar[armA=.2]{A1}{A2}
\ncbar[armA=0.6]{A2}{A}
\ncbar[armA=.2]{A}{B}
\ncbar[armA=0.8]{A1}{B}
\ncbar[armA=0.8]{B}{C}
%\ncbar[armA=.2]{A}{B}
\ncbar[armA=.2]{C}{D} 
\hspace{6mm}
\rnode{A7}{\Node{$\star$}}\rnode{A5}{\Node{$\star$}}\rnode{A6}{\Node{$\star$}}\rnode{A3}{\Node{$\star$}}\rnode{A1}{\Node{$\star$}}\rnode{A2}{\Node{$\star$}}\rnode{A}{\Node{$\star$}} \rnode{B}{\Node{$\star$}} \rnode{C}{\Node{$\star$}}
\rnode{D}{\Node{$\star$}} \rnode{D1}{\Node{$\dots$}} \rnode{D2}{\Node{$\star$}} \rnode{D3}{\Node{$\star$}}
\ncbar[armA=.2]{A7}{A5}
\ncbar[armA=.2]{A6}{A3}
\ncbar[armA=.2]{A1}{A2}
\ncbar[armA=0.6]{A2}{A}
\ncbar[armA=0.8]{A7}{A3}
\ncbar[armA=0.6]{A6}{A5}
\ncbar[armA=0.8]{A7}{A1}
\ncbar[armA=.2]{A}{B}
\ncbar[armA=0.8]{A7}{B}
\ncbar[armA=0.8]{B}{C}
%\ncbar[armA=.2]{A}{B}
\ncbar[armA=.2]{C}{D}  
\ncbar[armA=.2]{D2}{D3}
\caption{Irreducible
%which  the property that $\pi \vee \hat{0}_{[2r]}^2=1_{[2r]}.$ 
}
\label{fig:FiguraExemple1}
\end{center}
\end{figure} 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> formulas/involutiontypeIIIa.tex <==
%\usetikzlibrary{backgrounds}

\begin{tikzpicture}[scale=0.5]
\draw [white] (0,3.0) circle (0);

    \path [afill,thick] (2.0,0) rectangle (7.2,1.0);
\draw [thick] (0.7,0)--(0.7,1.6)--(7.9,1.6)--(7.9,0);
\draw [thick] (1.3,0)--(1.3,1.0)--(2.0,1.0);
\draw [dashed] (-1.8,1.6)--(10.3,1.6);

\node at (0.6,-0.5){$\pm X Y$};
\end{tikzpicture}

==> formulas/involutiontypeIIIb.tex <==
%\usetikzlibrary{backgrounds}

\begin{tikzpicture}[scale=0.5]
\draw [white] (0,3.0) circle (0);
    \path [afill,thick] (1.1,0) rectangle (6.3,1.0);
\draw [thick] (0.7,0)--(0.7,1.6)--(7.9,1.6)--(7.9,0);
\draw [thick] (7.2,0)--(7.2,1.0)--(6.3,1.0);
\draw [dashed] (-1.8,1.6)--(10.3,1.6);

\node at (7.2,-0.5){$\mp Y X$};
\end{tikzpicture}

==> formulas/notinneroddfig-pstricks.tex <==

 \begin{figure}[h]
\begin{center}
\vspace{1cm}
\psset{nodesep=3pt}
\psset{angle=90}

\rnode{A7}{\Node{$\star$}}\rnode{A5}{\Node{$\star$}}\rnode{A6}{\Node{$\star$}}\rnode{A3}{\Node{$\star$}}\rnode{A1}{\Node{$\star$}}\rnode{A2}{\Node{$\star$}}\rnode{A}{\Node{$\star$}} \rnode{B}{\Node{$\star$}} \rnode{C}{\Node{$\star$}}
\rnode{D}{\Node{$\star$}} \rnode{D1}{\Node{$\star$}} \rnode{D5}{\Node{$\star$}} \rnode{D2}{\Node{$\star$}} \rnode{D3}{\Node{$\star$}} \rnode{F1}{\Node{$\star$}} \rnode{F2}{\Node{$\star$}} \rnode{F3}{\Node{$\star$}} \rnode{F4}{\Node{$\star$}}
\ncbar[armA=.2]{A7}{A5}
\ncbar[armA=.2]{A6}{A3}
\ncbar[armA=.2]{A1}{A2}
\ncbar[armA=0.6]{A2}{A}
\ncbar[armA=0.6]{A5}{A6}
\ncbar[armA=0.6]{A3}{A1}
\ncbar[armA=.2]{A}{B}
\ncbar[armA=.2]{D1}{D5}


\ncbar[armA=1]{A7}{B}
\ncbar[armA=1]{B}{D3}
%\ncbar[armA=.2]{A}{B}
\ncbar[armA=.2]{C}{D}  
\ncbar[armA=.2]{D2}{D3}
\ncbar[armA=.2]{F1}{F2}
\ncbar[armA=.2]{F3}{F4}
\ncbar[armA=.6]{F2}{F3}
\ncbar[armA=1]{F1}{F4}
\ncbar[armA=1]{F1}{D3}

\caption{No irreducible }
\label{fig:FiguraExemple2}
\end{center}
\end{figure} 


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> formulas/pi112233_1.tex <==
\begin{picture}(32,3.5)(1,0)
{
  \linethickness{\thick}
  \put(2,0){\line(0,1){4.5}}
  \put(8,0){\line(0,1){4.5}}
}
\put(14,0){\line(0,1){4.5}}
\put(20,0){\line(0,1){4.5}}
\put(26,0){\line(0,1){4.5}}
\put(32,0){\line(0,1){4.5}}
{
  \linethickness{\thick}
  \put(2,4.5){\line(1,0){6}}
}
\put(14,4.5){\line(1,0){6}}
\put(26,4.5){\line(1,0){6}}
\end{picture}

==> formulas/pi112233_2.tex <==
\begin{picture}(32,3.5)(1,0)
\put(2,0){\line(0,1){4.5}}
\put(8,0){\line(0,1){4.5}}
{
  \linethickness{\thick}
  \put(14,0){\line(0,1){4.5}}
  \put(20,0){\line(0,1){4.5}}
}
\put(26,0){\line(0,1){4.5}}
\put(32,0){\line(0,1){4.5}}
\put(2,4.5){\line(1,0){6}}
{
  \linethickness{\thick}
  \put(14,4.5){\line(1,0){6}}
}
\put(26,4.5){\line(1,0){6}}
\end{picture}

==> formulas/pi112233_3.tex <==
\begin{picture}(32,3.5)(1,0)
\put(2,0){\line(0,1){4.5}}
\put(8,0){\line(0,1){4.5}}
\put(14,0){\line(0,1){4.5}}
\put(20,0){\line(0,1){4.5}}
{
  \linethickness{\thick}
  \put(26,0){\line(0,1){4.5}}
  \put(32,0){\line(0,1){4.5}}
}
\put(2,4.5){\line(1,0){6}}
\put(14,4.5){\line(1,0){6}}
{
  \linethickness{\thick}
  \put(26,4.5){\line(1,0){6}}
}
\end{picture}

==> formulas/sp111221a.tex <==
%latex kernelSetPartition [1,1,1,2,2,1,1]
\begin{picture}(38,6.5)(1,0)
\put(2,0){\line(0,1){7.5}}
\put(8,0){\line(0,1){7.5}}
\put(14,0){\line(0,1){7.5}}
\put(16,0){$\cdots$}
%\put(20,0){\line(0,1){4.5}}
%\put(26,0){\line(0,1){4.5}}
\put(32,0){\line(0,1){7.5}}
\put(38,0){\line(0,1){7.5}}
%\put(20,4.5){\line(1,0){6}}
\put(2,7.5){\line(1,0){36}}
\end{picture}
